The Role of Redundant Bases and Shrinkage Functions in Image Denoising

Wavelet denoising is a classical and effective approach for reducing noise in images and signals. Suggested in 1994, this approach is carried out by rectifying the coefficients of a noisy image in the transform domain, using a set of scalar shrinkage function (SFs). A plethora of papers deals with the optimal shape of the SFs and the transform used, where it is known that applying the SFs in redundant bases provides improved results. This paper provides a complete picture of the interrelations between the transform used, the optimal shrinkage functions, and the domains in which they are optimized. In particular, we show that for subband optimization, where each SF is optimized independently for a particular band, optimizing the SFs in the spatial domain is always better than or equal to optimizing the SFs in the transform domain. For redundant bases, we provide the expected denoising gain we may achieve, relative to the unitary basis, as a function of the redundancy rate.

==> leftOver.tex <==
\newpage
\section{left over - consider omitting}
Let $\Delta_i(\psi ~|~ W)$ denotes the error defined by method $i$, $i=1..3$, when applying the unitary transform $W$. Similarly $\Delta_i(\psi ~|~ U)$ denotes the respective error in the appropriate un-decimated transform $U$.

The following theorem states that optimizing the SFs using method~1 in the unitary
basis or in the un-decimated bases does not change the results.
\begin{theorem}
For each $\psi \in \Psi$,
$$
\Delta_1(\psi ~|~ W) = \Delta_1(\psi ~|~ U)
$$
\end{theorem}


%So far we have proven the relations marked in red in Figure
%\ref{fig:relations}. Now We are going to prove the relation marked
%in blue.
%
%\begin{figure}[tbh]
%\centering{\
% \psfig{figure=Figures/relations.eps,width=0.5\textwidth}
% \caption{\label{fig:relations} Relations.}}
%\end{figure}


%Denote the original deviation by  $\d$:
%$$
%\d = \x - \y
%$$
%Assume the cycle-spinning bases composed of $N$ unitary transforms
%whose bases are shifted versions, i.e.:
%$$
%W=\frac{1}{\sqrt{k}} \left [
%\begin{array}{c}
%W_1 \\
%W_2 \\
%\vdots \\
%W_k
%\end{array}
%\right ]
%$$
%Since each  $W_i$ is unitary we have:
%$$
%W^T W = I
%$$

{\bf Proof:}  \\
Denote by $\d$ the original deviation
$$
\d = \x - \y
$$
Each unitary transform preserves the original deviation:
$$
\d_i = W_i(\x-\y) = W_i \d  ~~~~\mbox{satisfying (following Eq. \ref{eq:uni})}~~\| \d_i \|^2 = \|
\d \|^2
$$
%We also define
%$$
%\p_i = \frac{1}{\sqrt{k}} W_i \d =  \frac{1}{\sqrt{k}} \d_i
%~~\Longrightarrow~ \| \p_i \|^2 = \frac{1}{{k}} \| \d_i
%\|^2=\frac{1}{{k}} \| \d \|^2 ~~\Longrightarrow~ \sum_i \| \p_i \|^2
%= \| \d \|^2
%$$
Similarly,
$$
U \d = \frac{1}{\sqrt{N}} \sum_i W_i \d = \frac{1}{\sqrt{N}} \sum_i \d_i
~~~~\mbox{satisfying (following Eq. \ref{eq:tight1})}~~ \| U \d \|^2 = \| \d \|^2
$$

Thus, the  deviation in the transform domain {\bf before} denoising
is equal to the deviation in the signal domain.
We now prove that the deviation in the signal domain {\bf after} denoising
in redundant bases is smaller or equal to the deviation after
denoising in a single unitary bases.

Define:
$$
\hat \d_i = (W_i \x - \psi \{ W_i \y \} ) ~~~\forall ~i
$$

%Assumptions 1:
%$$
%\| \hat \d_i \|^2 \leq \| \d_i \|^2 = \| \d \|^2
%$$
Due to the stationary property of natural images we assume:
\begin{equation}
\label{eq:di}
\| \hat \d_i \|^2 = \| \hat \d_j \|^2 = \Delta^2 ~~~~ \forall ~i,j
\end{equation}
Note that $\Delta^2$ is also the expected deviation in the unitary
case (where we choose only, say $W_1$ as the unitary transform).

Using the above assumption we have:
$$
\hat \d_u = ( U \x - \psi \{ U \y \}) = \frac{1}{\sqrt{N}}
\left (
\begin{array}{c}
\hat \d_1 \\
\hat \d_2 \\
\vdots \\
\hat \d_N
\end{array}
\right )
 ~~~~\mbox{satisfying (following Eq. \ref{eq:di}) }~~\| \hat \d_u \|^2 = \Delta^2
$$
Calculating the deviation in the spatial domain after denoising, we get:
$$
\hat \d = U^T \hat \d_u
$$
Following Equation~\ref{eq:tight2}  we have:
$$
\|  \hat \d \|^2 = \| U^T \hat \d_u \|^2 \leq  \| \hat \d_u \|^2 = \Delta^2
$$
Thus, the deviation in the spatial domain is smaller than what we have gotten
if applying denoising using unitary transform. Q.E.D.

%$$
%\| \hat \d \|^2 \leq \| \hat \p \|^2 = \| \hat \p_1 \|^2 + \| \hat
%\p_2 \|^2 + \cdots + \| \hat \p_k \|^2
% = \frac{1}{k} \sum_i^k \| \hat \d_i \|^2 = \Delta^2 ~~~QED
%$$

Conclusion:
$\psi^1_W=\psi^1_U$ and
$$
\Delta(\psi^1_W | U) = \Delta(\psi^1_U | U)
$$
\begin{theorem}
$$
\| U^T \psi\{ U \y \} - \x \|^2   \leq \| W^T \psi\{ W \y \} - \x \|^2   ~~~\forall ~\psi
$$
\end{theorem}


Accordingly, we define
$$
\hat \psi^i_W = \arg \min_{\psi \in \Psi} \Delta_i(\psi ~|~ W)  ~~\mbox{and}~~
\hat \psi^i_U = \arg \min_{\psi \in \Psi} \Delta_i(\psi ~|~ U) .
$$



==> shrinkage.tex <==
\section{Inequalities and Bounds}

Define:
\begin{equation}
\label{def:pk} \p_k = \arg \min_{\p} \Delta_k(\p) ~~~k \in \{1,2,3\}
\end{equation}

Since we proved that
\begin{equation}
\label{eq:ineq1} \Delta_3 (\p) \leq \Delta_2 (\p)  \leq \Delta_1
(\p)
\end{equation}
for each given $\p$, it follows that:
\begin{equation}
\label{eq:ineq2} \Delta_3(\p_3) \leq \Delta_2(\p_2) \leq
\Delta_1(\p_1)
\end{equation}

{\bf Proof:} We first prove the left inequality. From from the
definition \ref{def:pk} we know that $\p_3$ minimizes $\Delta_3$,
thus, $\Delta_3 (\p_3) \leq \Delta_3 (\p_2)$. However, from
Eq.~\ref{eq:ineq1} we have that $\Delta_3 (\p_2) \leq \Delta_2
(\p_2)$ from which it readily follows  that $\Delta_3 (\p_3) \leq
\Delta_2 (\p_2)$.
The second inequality can be shown using a similar reasoning. Q.E.D. \\

The last theorem  provide the justification for optimizing the SFs
using methods 2 and 1. It shows that the penalty functions used in
these methods serve as upper bounds for the desired penalty (method
3) that might be difficult to achieve. Thus, minimizing the upper
bounds, also minimizes the desired penalty function, although the
results might not be the optimal one. Note also, that according to
the proof above, the actual errors using methods 2 and 1 are even
tighter, i.e.:
\begin{eqnarray}
\Delta_3(\p_3) \leq \Delta_3(\p_2) \leq \Delta_2(\p_2) ~~~\mbox{for method 2}\\
\Delta_3(\p_3) \leq \Delta_3(\p_1) \leq \Delta_2(\p_1) ~~~\mbox{for
method 1}
\end{eqnarray}
Nevertheless, it can not be assured that the actual error for $\p_2$
outperforms the actual error of $\p_1$, i.e. the relation:
$$
\Delta_3(\p_2) \leq \Delta_3(\p_1)
$$
is not necessarily true. To see this remember that $\Delta_3=\sum_i
\Delta_2^i$ where $i$ runs over the various bands. This can be
interpreted as a projection of the vector $\Delta_2$ onto a vector
of ones denoted by $\bf 1$. Thus,
$$
 \Delta_3(\p_2) = {\bf 1}^T \Delta_2(\p_2) ~~\mbox{and}~~
 \Delta_3(\p_1) = {\bf 1}^T \Delta_2(\p_1)
$$
Although the magnitudes $\| \Delta_2(\p_2) \|^2 \leq \|
\Delta_2(\p_1) \|^2$, the projections onto the vector $\bf 1$ does
not necessarily preserves the order of magnitudes. Nevertheless,
this is true on the average case if we assume that $\Delta_2(\p_2)$
and $\Delta_2(\p_1)$ are randomly distributed.

\begin{figure}[tbh]
\centering{\
 \psfig{figure=Figures/deltas.eps,width=0.7\textwidth}
 \caption{\label{fig:deltas} Comparison definitions.}}
\end{figure}

